The use of Semantic Technologies in Computer Science Curriculum: A Systematic Review

Semantic technologies are evolving and being applied in several research areas, including the education domain. This paper presents the outcomes of a systematic review carried out to provide an overview of the application of semantic technologies in the context of the Computer Science curriculum and discuss the limitations in this field whilst offering insights for future research. A total of 4,510 studies were reviewed, and 37 were analysed and reported. As a result, while semantic technologies have been increasingly used to develop Computer Science curricula, the alignment of ontologies and accurate curricula assessment appears to be the most significant limitations to the widespread adoption of such technologies.

==> table/knowledge_rep.tex <==
\begin{tabular}{|c|c|c|} 
\hline
\textbf{Class}                            & \textbf{Subcalssof} & \textbf{Description}     \\ 
\hline
BodyOfKnowledge & owl:Thing  & \makecell[c]{A body of knowledge is the complete set of \\concepts, terms and activities that make up \\a professional domain.}
\\
\hline
KnowledgeArea   & owl:Thing  & \makecell[c]{Knowledge areas are areas of specialization. \\The CS2013 Body of Knowledge is presented as a set of Knowledge Areas (KAs), \\organized on topical themes rather than by course boundaries.}
\\
\hline
KnowledgeUnit   & owl:Thing  & \makecell[c]{In CS2013, Knowledge Areas are composed of Knowledge \\Units. Each KA is further organised into a set \\of Knowledge Units (KUs), which are summarized \\in a table at the head of each KA section.}
\\
\hline
Topic           & owl:Thing  & \makecell[c]{In CS2013, Topics are identified 
as either \\“Core” or “Elective” with the core further \\subdivided into “Tier-1” and “Tier-2.”.}              
\\
\hline
Core-Tier1       & Topic      & \makecell[c]{A Core Tier-1 topic should be a required \\part of every Computer Science curriculum.}                                          
\\
\hline
Core-Tier2       & Topic      & \makecell[c]{Core Tier-2 topics are generally essential \\in an undergraduate computer-science degree.}
\\
\hline
Course           & owl:Thing  & \makecell[c]{a course is a unit of teaching \\that typically lasts one academic term, is led by one or more instructors\\,~and has a fixed roster of students.}
\\
\hline
\end{tabular}

==> table/similarity_comparison.tex <==

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Approach}     & \textbf{Techniques}  & \textbf{Papers}        \\
\hline
Term-based      &Cosine Similarity; K-means &\cite{Orellana2018,Pawar2018,Adrian2020,Seidel2020,Wang2019,Saquicela2018SimilarityDA}            \\
\hline
Corpus-based    & Latent Semantic Analysis  &\cite{Orellana2018} \cite{Pawar2018} \cite{Adrian2020} \cite{Fiallos2018}           \\
\hline
knowledge-based     &Synsets; Max Similarity  &\cite{Nuntawong2016} \cite{Pawar2018} \cite{Nuntawong2017}       \\
\hline
\end{tabular}
